When Should Models Change Their Minds? Contextual Belief Management in Large Language Models

Long-horizon interactions require language models to manage accumulating information: when to update their state, when to preserve their state, and what to ignore. We study this challenge as Contextual Belief Management (CBM): maintaining a predicted belief state aligned with formal evidence while isolating task-irrelevant noise. To make CBM measurable, we introduce BeliefTrack, a closed-world benchmark spanning Rule Discovery and Circuit Diagnosis, where a finite belief space and symbolic verifiers enable exact turn-level evaluation. BeliefTrack diagnoses three failures: Failed Stay, Failed Update, and Failed Isolation. Across multiple LLMs, vanilla models exhibit severe CBM failures, while explicit belief-tracking prompts provide limited gains. In contrast, reinforcement learning with belief-state rewards reduces failure rates by 70.9% on average. Further probing reveals latent belief-state dynamics behind these failures, and representation-level steering reduces failure rates by 46.1% across two tasks (Code is available at https://github.com/zjunlp/CBM).

==> tables/hyperparameters.tex <==
\begin{table}[htbp]
\centering
\small
\setlength{\tabcolsep}{1.5pt}
\renewcommand{\arraystretch}{0.9}
\caption{
Implementation parameters grouped by RL training hyperparameters and sampling hyperparameters.
Batch Size denotes the total training batch size computed as \texttt{per\_device\_train\_batch\_size} $\times$ \texttt{num\_devices}.
}
\begin{tabular}{lcc}
\toprule
\textbf{Parameter} & \textbf{Qwen2.5-7B} & \textbf{Qwen3.5-9B} \\
\midrule

\multicolumn{3}{l}{\textbf{RL Hyperparameters}} \\
Batch Size & 8 & 4 \\
Gradient Accumulation Steps & 4 & 4 \\
Number of Generations & 8 & 8 \\
Learning Rate & 1e-4 & 1e-4 \\
KL Coefficient & 0.04 & 0.04 \\
Importance Sampling & token-level & token-level \\
Task-A-Training-Steps & 500 & 520 \\
Task-B-Training-Steps & 374 & 338 \\
LoRA Rank & 16 & 16 \\
LoRA Alpha & 32 & 32 \\
LoRA Dropout & 0.05 & 0.05 \\
Target Modules & all-linear & all-linear \\
\midrule

\multicolumn{3}{l}{\textbf{Sampling Hyperparameters}} \\
Rollout Temperature & 0.3 & 1.0 \\
Rollout Top-$p$ & default & 1.0 \\
Rollout Top-$k$ & default & 20 \\
Presence Penalty & default & 1.5 \\
Repetition Penalty & default & 1.0 \\
Evaluation Temperature & 0.3 & 1.0 \\
Probing Temperature & -- & 0.0 \\

\bottomrule
\end{tabular}
\label{tab:impl_params}
\end{table}

==> tables/main.tex <==
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.12}
\definecolor{idcolor}{HTML}{E8F0FE}
\definecolor{oodcolor}{HTML}{FCE8E6}

\newcommand{\id}[1]{\cellcolor{idcolor}#1}
\newcommand{\ood}[1]{\cellcolor{oodcolor}#1}

\newcommand{\val}[1]{\makebox[4.5em][l]{#1}}

\newcommand{\Bpos}[1]{\ensuremath{{}_{\scriptscriptstyle \textcolor{teal}{\downarrow #1\%}}}}
\newcommand{\Bneg}[1]{\ensuremath{{}_{\scriptscriptstyle \textcolor{purple}{\uparrow #1\%}}}}
\newcommand{\Gpos}[1]{\ensuremath{{}_{\scriptscriptstyle \textcolor{teal}{\uparrow #1\%}}}}
\newcommand{\Gneg}[1]{\ensuremath{{}_{\scriptscriptstyle \textcolor{purple}{\downarrow #1\%}}}}

\small
\begin{tabular}{lcccccccc}
\toprule
\multirow{2}{*}{\textbf{Method}}
  & \multicolumn{3}{c}{\textbf{Rule Discovery (RD)}}
  & \multicolumn{3}{c}{\textbf{Circuit Diagnosis (CD)}}
  & \multicolumn{2}{c}{\textbf{General}} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-9}
  & \textbf{FSR} $\downarrow$
  & \textbf{FUR} $\downarrow$
  & \textbf{FIR} $\downarrow$
  & \textbf{FSR} $\downarrow$
  & \textbf{FUR} $\downarrow$
  & \textbf{FIR} $\downarrow$
  & \textbf{GSM8K} $\uparrow$
  & \textbf{MMLU} $\uparrow$ \\
\midrule

\rowcolor{black!8}
\multicolumn{9}{l}{\textbf{Qwen2.5-7B-Instruct}} \\

Vanilla
  & \val{99.0}
  & \val{98.0}
  & \val{97.0}
  & \val{99.0}
  & \val{98.0}
  & \val{97.0}
  & \val{83.3 $\pm$ 0.4}
  & \val{73.5 $\pm$ 0.3} \\

BT-Prompt
  & \val{79.0\Bpos{20.2}}
  & \val{80.0\Bpos{18.4}}
  & \val{95.0\Bpos{2.1}}
  & \val{48.0\Bpos{51.5}}
  & \val{87.9\Bpos{10.3}}
  & \val{92.0\Bpos{5.2}}
  & \val{---}
  & \val{---} \\

RL-RD
  & \id{\val{\textbf{0.0}\Bpos{100.0}}}
  & \id{\val{\textbf{2.0}\Bpos{98.0}}}
  & \ood{\val{\textbf{20.0}\Bpos{79.4}}}
  & \ood{\val{\underline{6.0}\Bpos{93.9}}}
  & \ood{\val{\underline{28.3}\Bpos{71.1}}}
  & \ood{\val{\underline{35.0}\Bpos{63.9}}}
  & \val{84.8 $\pm$ 0.5}
  & \val{73.1 $\pm$ 0.2} \\

RL-CD
  & \ood{\val{\underline{42.0}\Bpos{57.6}}}
  & \ood{\val{\underline{74.0}\Bpos{24.5}}}
  & \ood{\val{\underline{57.0}\Bpos{41.2}}}
  & \id{\val{\textbf{0.0}\Bpos{100.0}}}
  & \id{\val{\textbf{0.0}\Bpos{100.0}}}
  & \ood{\val{\textbf{20.0}\Bpos{79.4}}}
  & \val{83.9 $\pm$ 0.3}
  & \val{73.4 $\pm$ 0.4} \\

\midrule

\rowcolor{black!8}
\multicolumn{9}{l}{\textbf{Qwen3.5-9B}} \\

Vanilla
  & \val{47.0}
  & \val{60.0}
  & \val{83.7}
  & \val{43.2}
  & \val{62.7}
  & \val{95.4}
  & \val{94.0 $\pm$ 0.2}
  & \val{78.1 $\pm$ 0.3} \\

BT-Prompt
  & \val{49.0\Bneg{4.3}}
  & \val{69.0\Bneg{15.0}}
  & \val{81.4\Bpos{2.7}}
  & \val{47.4\Bneg{9.7}}
  & \val{63.5\Bneg{1.3}}
  & \val{81.4\Bpos{14.7}}
  & \val{---}
  & \val{---} \\

RL-RD
  & \id{\val{\textbf{6.0}\Bpos{87.2}}}
  & \id{\val{\textbf{8.0}\Bpos{86.7}}}
  & \ood{\val{\textbf{18.6}\Bpos{77.8}}}
  & \ood{\val{\underline{20.0}\Bpos{53.7}}}
  & \ood{\val{\underline{21.4}\Bpos{65.9}}}
  & \ood{\val{\underline{34.9}\Bpos{63.4}}}
  & \val{94.5 $\pm$ 0.6} 
  & \val{78.2 $\pm$ 0.3} \\

RL-CD
  & \ood{\val{\underline{31.0}\Bpos{34.0}}}
  & \ood{\val{\underline{34.0}\Bpos{43.3}}}
  & \ood{\val{\underline{41.9}\Bpos{49.9}}}
  & \id{\val{\textbf{12.1}\Bpos{72.0}}}
  & \id{\val{\textbf{15.9}\Bpos{74.6}}}
  & \ood{\val{\textbf{16.3}\Bpos{82.9}}}
  & \val{94.5 $\pm$ 0.6}
  & \val{78.7 $\pm$ 0.3} \\

\bottomrule
\end{tabular}
\vspace{-0.5em}
\caption{
Main diagnostic and cross-task generalization results.
We report Failed Stay Rate (FSR), Failed Update Rate (FUR), and Failed Isolation Rate (FIR) (lower is better $\downarrow$), together with MMLU and GSM8K accuracy (higher is better $\uparrow$).
\textbf{Bold} and \underline{underline} denote the \textbf{best} and \underline{second-best} results respectively.
\textbf{RL-RD} and \textbf{RL-CD} indicate models trained solely on Rule Discovery or Circuit Diagnosis.
\protect\colorbox{idcolor}{Blue} and \protect\colorbox{oodcolor}{orange} indicate in-domain (ID) and out-of-domain (OOD) generalization, respectively.
Subscripts show relative changes from Vanilla.}
\label{tab:main}
\vspace{-0.6em}
\end{table*}


==> tables/noise_controls.tex <==
\begin{table}[t]
  \centering
  \small
  \setlength{\tabcolsep}{12pt}
  \renewcommand{\arraystretch}{1.08}
  \begin{tabular}{lc}
  \toprule
  \textbf{Condition} & \textbf{FIR} $\downarrow$ \\
  \midrule
  Correct hint & 46.51 \\
  Neutral filler & 72.09 \\
  Random wrong hint & 74.42 \\
  Framed authority hint & \textbf{90.70} \\
  \bottomrule
  \end{tabular}
  \caption{
  Noise-intervention control study.
  We compare matched intervention variants to separate the effect of framing from added context length and hint presence.
  The framed authority hint yields the highest FIR, indicating stronger disruption of belief isolation.
  }
  \label{tab:noise_controls}
  \end{table}

